Acceleration and radiation: Classical and quantum aspects

It has been known for some time that the classical concept of radiation is not covariant: for uniformly accelerated particles, it depends on the state of motion of the observer relative to the particle emitting it. Moreover, recent literature in the field of Quantum Field Theory in Curved Spacetimes suggests a deep connection between bremsstrahlung and the Unruh effect, where zero-Rindler energy particles have played a central role beyond constructing the radiation contents of systems; as this is an unfamiliar concept, it seems unsettling to deal with particles having no energy. This thesis studies such a connection in both the classical and quantum perspectives, showing how the quantum Unruh effect is responsible for the classical radiation detected for the electric and gravitational cases, and studies the role of zero-Rindler-energy particles and how they relate to the radiative field of uniformly accelerated particles.

==> frontmatter/glossaries.tex <==
\makeglossaries



\newglossaryentry{formula}
{
        name=formula,
        description={A mathematical expression}
}

\newacronym[]{qftcs}{QFTCS}{Quantum Field Theory in Curved Spacetimes}

\newacronym[]{fdu}{FDU}{Fulling-Davies-Unruh}

\newacronym[]{fduthermal}{FDU thermal bath}{Fulling-Davies-Unruh thermal bath}

==> frontmatter/my-cover.tex <==
% !TeX root = ../thesis-Portales.tex

\setcounter{page}{-1}

\thispagestyle{empty}

\null 

\vfill

\begin{flushleft}
    \begin{Huge}
        \textbf{\textsf{Acceleration and Radiation: \\[6pt] Classical and Quantum Aspects}}
    \end{Huge}

    \vspace{.5cm}

    \begin{Large}
        \textsc{Felipe Ignacio Portales Oliva}\\[7pt]
    \end{Large}

    \hrule
    \vspace{1cm}
    
    \begin{minipage}[b]{.58\textwidth}
        Advisor: Dr. André G. S. Landulfo
        \\
        Santo André, São Paulo, Brazil -- 2023
    \end{minipage}
    \hfill 
    % \includegraphics[width=.3\textwidth]{./images/logotipo-ufabc-lateral.png}
    \includegraphics[width=.3\textwidth]{./images/logo-variacao3-fundo-claro.png}
\end{flushleft} 
